Fast and Optimal Differentially Private Frequent-Substring Mining

Given a dataset of $n$ user-contributed strings, each of length at most $\ell$, a key problem is how to identify all frequent substrings while preserving each user's privacy. Recent work by Bernardini et al. (PODS'25) introduced a $\varepsilon$-differentially private algorithm achieving near-optimal error, but at the prohibitive cost of $O(n^2\ell^4)$ space and processing time. In this work, we present a new $\varepsilon$-differentially private algorithm that retains the same near-optimal error guarantees while reducing space complexity to $O(n \ell+ |\Sigma| )$ and time complexity to $O(n \ell\log |\Sigma| + |\Sigma| )$, for input alphabet $\Sigma$. Our approach builds on a top-down exploration of candidate substrings but introduces two new innovations: (i) a refined candidate-generation strategy that leverages the structural properties of frequent prefixes and suffixes, and (ii) pruning of the search space guided by frequency relations. These techniques eliminate the quadratic blow-ups inherent in prior work, enabling scalable frequent substring mining under differential privacy.

==> macro.tex <==
%% BEGIN OF USER-DEFINED

\makeatletter

% Format: \@ifundefined{environment_name}{definition}{action_if_already_defined}

\@ifundefined{theorem}{\newtheorem{theorem}{Theorem}[section]}{}
\@ifundefined{proposition}{\newtheorem{proposition}{Proposition}[section]}{}
\@ifundefined{lemma}{\newtheorem{lemma}[theorem]{Lemma}}{}
\@ifundefined{remark}{\newtheorem{remark}[theorem]{Remark}}{}
\@ifundefined{problem}{\newtheorem{problem}[theorem]{Problem}}{}
\@ifundefined{notation}{\newtheorem{notation}[theorem]{Notation}}{}
\@ifundefined{example}{\newtheorem{example}[theorem]{Example}}{}
\@ifundefined{definition}{\newtheorem{definition}[theorem]{Definition}}{}
\@ifundefined{observation}{\newtheorem{observation}[theorem]{Observation}}{}
\@ifundefined{corollary}{\newtheorem{corollary}[theorem]{Corollary}}{}
\@ifundefined{claim}{\newtheorem{claim}[theorem]{Claim}}{}
\@ifundefined{fact}{\newtheorem{fact}[theorem]{Fact}}{}
\@ifundefined{conj}{\newtheorem{conj}[theorem]{Conjecture}}{}
\@ifundefined{assm}{\newtheorem{assm}[theorem]{Assumption}}{}

\makeatother

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{conj}[theorem]{Conjecture}
% \newtheorem{assm}[theorem]{Assumption}
% \newtheorem{comment}[theorem]{Comment}
\newenvironment{sproof}{%
  \renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}

\renewenvironment{quote}
  {\list{}{\rightmargin=0.3cm \leftmargin=0.3cm}%
   \item\relax}
  {\endlist}

%\renewcommand{\algorithmicprocedure}{\textbf{Procedure}}
%\renewcommand{\algorithmicrequire}{\quad\enspace\;\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\quad\enspace\;\textbf{Ensure:}}


%mathcal
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%mathscr
\newcommand{\sA}{\mathscr{A}}
%pmb
\newcommand{\pmba}{\pmb{a}}
\newcommand{\pmbb}{\pmb{b}}
\newcommand{\pmbc}{\pmb{c}}
\newcommand{\pmbe}{\pmb{e}}
\newcommand{\pmbf}{\pmb{f}}
\newcommand{\pmbp}{\pmb{p}}
\newcommand{\pmbs}{\pmb{s}}
\newcommand{\pmbu}{\pmb{u}}
\newcommand{\pmbv}{\pmb{v}}
\newcommand{\pmbx}{\pmb{x}}
\newcommand{\pmby}{\pmb{y}}
\newcommand{\pmbz}{\pmb{z}}
\newcommand{\pmbpi}{\pmb{\pi}}
\newcommand{\pmbPhi}{\pmb{\Phi}}
\newcommand{\pmbnu}{\pmb{\nu} }
\newcommand{\pmbomega}{\pmb{\omega}}
%mathds
% \newcommand{\dsone}{\mathds{1}}
%mathfrak
\newcommand{\mfrkP}{\mathfrak{P}}
\newcommand{\mfrkM}{\mathfrak{M}}
%mathrm
\newcommand{\mrmA}{\mathrm{A}}
\newcommand{\mrmM}{\mathrm{M}}
\newcommand{\mrmH}{\mathrm{H}}
%mathbb
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\mbbS}{\mathbb{S}}
\newcommand{\mbbU}{\mathbb{U}}
\newcommand{\mbbZ}{\mathbb{Z}}
\newcommand{\Z}{\mathbb{Z}}
%mathbf
\newcommand{\mbfA}{\mathbf{A}}
\newcommand{\mbfC}{\mathbf{C}}
\newcommand{\mbfD}{\mathbf{D}}
\newcommand{\mbfP}{\mathbf{P}}
\newcommand{\mbfS}{\mathbf{S}}
\newcommand{\mbfX}{\mathbf{X}}
\newcommand{\mbfZ}{\mathbf{Z}}

%opreators
\newcommand{\poly}[1]{\ensuremath{\texttt{poly}#1}\xspace}
\newcommand{\intint}[2]{\llbracket #1, #2 \rrbracket}
\newcommand{\rangeint}[2]{\{#1, \ldots, #2\}}
\newcommand{\range}[1]{\mathbb{N}_{< {#1}}}
\newcommand{\zeroton}[1]{\mathbb{N}_{\le {#1}}}
% \newcommand\naturalNumbersZeroToUpN[1]{\mathbb{N}_{\le {#1}}}
\newcommand\clamp[3]{\text{clamp} \bracket{ {#1}, {#2}, {#3} } }
\newcommand{\TVDISTANCE}[2]{\mathds{TV} \left( {#1} ,\, {#2} \right)}
\newcommand{\tvdistance}[2]{\mathds{TV} ( {#1} ,\, {#2} )}
\newcommand{\fdivergence}[2]{\mathds{D}_f \left( {#1} ,\, {#2} \right)}
\newcommand{\norm}[1]{\lVert {#1} \rVert}
\newcommand{\NORM}[1]{\left\lVert {#1} \right\rVert}
\newcommand{\bignorm}[1]{\big\lVert {#1} \big\rVert}
\DeclareMathOperator{\mathsign}{sgn}
\newcommand{\sgn}[1]{\mathsign \left( {#1} \right)}
\newcommand{\PAREN}[1]{{\left( {#1} \right)}}
\newcommand{\Biggparen}[1]{{\Bigg( {#1} \Bigg)}}
\newcommand{\Bigparen}[1]{{\Big( {#1} \Big)}}
\newcommand{\bigparen}[1]{{\big( {#1} \big)}}
\newcommand{\paren}[1]{{( {#1} )}}
\newcommand{\floor}[1]{{\lfloor {#1} \rfloor}}
\newcommand{\ceil}[1]{{\lceil {#1} \rceil}}
\newcommand{\CEIL}[1]{{\left\lceil {#1} \right\rceil}}
\newcommand{\angles}[1]{{\langle {#1} \rangle}}
\newcommand{\bracket}[1]{{[ {#1} ]}}
\newcommand{\BigBracket}[1]{{\big[ {#1} \big]}}
\newcommand{\BRACKET}[1]{{\left[ {#1} \right]}}
\newcommand{\CARD}[1]{\left| {#1} \right|}
\newcommand{\card}[1]{\lvert {#1} \rvert}
\newcommand{\SET}[1]{\left\{ {#1} \right\}}
\newcommand{\set}[1]{\{ {#1} \}}
\newcommand{\eps}{\varepsilon}
\newcommand{\tildeeps}{\tilde{\varepsilon}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\Probability}{\mathbb{P}}
\NewDocumentCommand\p{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\Pr [ #1 ]}
    {\Pr_{#1}[#2]}
  }
}
\RenewDocumentCommand\P{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\Pr \left[#1\right]}
    {\Pr_{#1}\left[#2\right]}
  }
}
\DeclareMathOperator*{\Expectation}{\mathbb{E}}
\NewDocumentCommand\E{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\Expectation \left[#1\right]}
    {\Expectation_{#1}\left[#2\right]}
  }
}
\DeclareMathOperator*{\Variance}{\mathbb{V}\mathrm{ar}}
\NewDocumentCommand\Var{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\Variance \left[#1\right]}
    {\Variance_{#1}\left[#2\right]}
  }
}

\NewDocumentCommand\GammaDist{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\operatorname{\mathcal{G}amma}\left( {#1} \right)}
    {\operatorname{\mathcal{G}amma}\left( {#1}, {#2} \right)}
  }
}

\NewDocumentCommand\LapNoise{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\operatorname{\mathbb{L}ap}\left( {#1} \right)}
    {\operatorname{\mathbb{L}ap}\left( {#1}, {#2} \right)}
    % {\operatorname{\mathcal{L}ap}\left( {#1} \right)}
    % {\operatorname{\mathcal{L}ap}\left( {#1}, {#2} \right)}
  }
}

\NewDocumentCommand\GumbelNoise{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\operatorname{\mathbb{G}umbel}\left( {#1} \right)}
    {\operatorname{\mathbb{G}umbel}\left( {#1}, {#2} \right)}
    % {\operatorname{\mathcal{G}umbel}\left( {#1} \right)}
    % {\operatorname{\mathcal{G}umbel}\left( {#1}, {#2} \right)}
  }
}

% \newcommand{\LapNoise}[2]{\mathcal{L}ap\left( {#1}, {#2} \right)}
% \newcommand{\GumbelNoise}[2]{\mathcal{G}umbel\left( {#1}, {#2} \right)}

%============Project Specific Commands====================



% \newcommand{\DataSet}{\mathcal{X}}
\newcommand{\DataSet}{\mathcal{D}}
% \newcommand{\Document}[1]{\mathcal{S}_{#1}}
\newcommand{\length}{\ell}
% \newcommand{\lengthprime}{\ell^{\mathsf{bit}}}
\newcommand{\lengthprime}{\ell_{\,\mathsf{bit}}}
\newcommand{\element}{i}
\newcommand{\user}{u}
\newcommand{\UserSet}{\mathcal{U}}
\newcommand{\UserData}[1]{x^{({#1})}}
\newcommand{\NeighborUserData}[1]{x'^{\,({#1})}}
\newcommand{\SortedUserData}[1]{y^{({#1})}}
\newcommand{\DataDomain}{\mathcal{D}}
\newcommand{\IntSet}[2]{[{#1}\,.\,.\,{#2}]}
\newcommand{\Binomial}[2]{\operatorname{\mathbb{B}in} ( {#1} , {#2} )}
\newcommand{\Bernoulli}[1]{\operatorname{\mathbb{B}ernoulli}\left( {#1} \right)}
\newcommand{\indicator}[1]{\mathds{1}_{\left[#1\right]}}
\newcommand\inner[2]{\left\langle #1, #2 \right\rangle}
%============Project Specific Commands====================

\newcommand{\algname}{\mathsf{DPFreqSub}}
\newcommand{\freqUpperBound}{\tau_{\top}}
\newcommand{\freqLowerBound}{\tau_{\bot}}
\NewDocumentCommand\Candidates{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\mathcal{C}}
    {\mathcal{C}_{#1}}
  }
}

\NewDocumentCommand\CandidateExtension{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\overline{\mathcal{C}}}
    {\overline{\mathcal{C}}_{#1}}
  }
}

\DeclareMathOperator\supp{\textsc{supp}}
\DeclareMathOperator\Set{\textsc{Set}}

\newcommand{\HeavyPaths}[1]{\mathsf{HP}(#1)}
% \newcommand{\Document}[1]{\mathcal{S}_{#1}}
\NewDocumentCommand\Document{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\mathcal{S}}
    {\mathcal{S}_{#1}}
  }
}


\NewDocumentCommand\hist{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\vec{h}}
    {\vec{h}\BRACKET{#1}}
  }
}

\NewDocumentCommand\noisyhist{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\Tilde{h}}
    {\Tilde{h}\BRACKET{#1}}
  }
}

\NewDocumentCommand\intermediateHist{ g }{
  \ensuremath{
    \IfNoValueTF{#1}
    {\hat{h}}
    {\hat{h}\BRACKET{#1}}
  }
}


\NewDocumentCommand\DiscreteLapNoise{ g g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {
        \IfNoValueTF{#1}
        {\operatorname{\mathbb{DL}ap}}
        {\operatorname{\mathbb{DL}ap}\left( {#1} \right)}
    }
    {\operatorname{\mathbb{DL}ap}\left( {#1}, {#2} \right)}
  }
}


\NewDocumentCommand\UniformNoise{ m g }{
  \ensuremath{
    \IfNoValueTF{#2}
    {\operatorname{\mathbb{U}niform}\left( {#1} \right)}
    {\operatorname{\mathbb{U}niform}\left( {#1}, {#2} \right)}
  }
}


\NewDocumentCommand{\occ}{m g}{%
  \IfNoValueTF{#2}
    {\ensuremath{\operatorname{occ}\paren{#1}}}
    {\ensuremath{\operatorname{occ}_{#2}\paren{#1}}}
}

\NewDocumentCommand{\freq}{m g}{%
  \IfNoValueTF{#2}
    {\ensuremath{f_{#1}}}                    % frequency of #1 alone
    {\ensuremath{f_{#1}\paren{#2}}} % frequency of #1 in #2
}

\NewDocumentCommand{\difffreq}{m g}{%
  \IfNoValueTF{#2}
    {\ensuremath{\Delta f_{#1}}}                    % frequency of #1 alone
    {\ensuremath{\Delta f_{#1}\paren{#2}}} % frequency of #1 in #2
}
\newcommand{\BTM}{\mathcal{M}_{\mathrm{BT}}}


\NewDocumentCommand{\freqnoisy}{m g}{%
  \IfNoValueTF{#2}
    {\ensuremath{\tilde{f}_{#1}}}                    % frequency of #1 alone
    {\ensuremath{\tilde{f}_{#1}\paren{#2}}} % frequency of #1 in #2
}

\newcommand{\laplacenoise}{\mathsf{Lap}}

\NewDocumentCommand{\noisyfreq}{m g}{%
  \IfNoValueTF{#2}
    {\ensuremath{\tilde{f}_{#1}}}                    % frequency of #1 alone
    {\ensuremath{\tilde{f}_{#1}\paren{#2}}} % frequency of #1 in #2
}

\newcommand{\substr}[1]{\ensuremath{\texttt{substr}(#1)}\xspace}
\newcommand{\suffix}[1]{\ensuremath{\texttt{suffix}(#1)}\xspace}


% ================== suffix tree-related  ==================

\newcommand{\startpos}[1]{\ensuremath{\texttt{start}(#1)}\xspace}
\newcommand{\str}[1]{\ensuremath{\texttt{str}(#1)}\xspace}
\newcommand{\locus}[1]{\ensuremath{\texttt{locus}(#1)}\xspace}
\newcommand{\parent}[2][]{\ensuremath{\texttt{parent}^{#1}(#2)}\xspace}
\newcommand{\depth}[1]{\ensuremath{\texttt{depth}(#1)}\xspace}
\newcommand{\child}[2]{\ensuremath{\texttt{child}(#1, #2)}\xspace}
\newcommand{\children}[1]{\ensuremath{\texttt{children}(#1)}\xspace}

\newcommand{\trieof}[1]{\ensuremath{\mathit{T}_{#1}}\xspace}
\newcommand{\suffixtreeof}[1]{\ensuremath{\mathit{ST}_{#1}}\xspace}

\newcommand{\trienode}[1]{\ensuremath{\texttt{node}(#1)}\xspace} % defined only for tries

% ================== end of suffix tree-related  ==================


\newif\ifcomment
\commenttrue
% \commentfalse

% \newif\ifsupp
% \supptrue


\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\ifcomment
\newcommand{\hao}[1]{\textcolor{blue}{[HAO: #1]}}
\newcommand{\peaker}[1]{\textcolor{black!50!green}{[Peaker: #1]}}
\newcommand{\rayne}[1]{\textcolor{purple}{[Rayne: #1]}}
\newcommand{\fix}[1]{\textcolor{red}{#1}}
\newcommand{\suggest}[1]{\textcolor{DarkGreen}{#1}}
\newcommand{\minoredit}[1]{\textcolor{DarkGreen}{#1}}
\else

% \def\@bsphack{%
%   \relax
%   \ifhmode
%     \@savsk\lastskip
%     \@savsf\spacefactor
%   \fi}
% \def\@esphack{%
%   \relax
%   \ifhmode
%     \spacefactor\@savsf
%     \ifdim\@savsk>\z@
%       \ignorespaces
%     \fi
% \fi}
\makeatletter
\newcommand{\hao}[1]{%
  \@bsphack
  \@esphack
}
\makeatother

% \newcommand{\hao}[1]{}

%\newcommand{\haoCameraReady}[1]{\textcolor{DarkGreen}{#1}}
% \newcommand{\haoCameraReady}[1]{#1}
\fi

%% END OF USER-DEFINED
